Connection Between the Circumgalactic Medium and the Interstellar Medium of Galaxies: Results from the COS-GASS Survey

We present a study exploring the nature and properties of the Circum-Galactic Medium (CGM) and its connection to the atomic gas content in the interstellar medium (ISM) of galaxies as traced by the HI 21cm line. Our sample includes 45 low-z (0.026-0.049) galaxies from the GALEX Arecibo SDSS Survey. Their CGM was probed via absorption in the spectra of background Quasi-Stellar Objects at impact parameters of 63 to 231kpc. The spectra were obtained with the Cosmic Origins Spectrograph aboard the Hubble Space Telescope. We detected neutral hydrogen (Ly$\alpha$ absorption-lines) in the CGM of 92% of the galaxies. We find the radial profile of the CGM as traced by the Ly$\alpha$ equivalent width can be fit as an exponential with a scale length of roughly the virial radius of the dark matter halo. We found no correlation between the orientation of sightline relative to the galaxy major axis and the Ly$\alpha$ equivalent width. The velocity spread of the circumgalactic gas is consistent with that seen in the atomic gas in the interstellar medium. We find a strong correlation (99.8% confidence) between the gas fraction (M(HI)/M*) and the impact-parameter-corrected Ly$\alpha$ equivalent width. This is stronger than the analogous correlation between corrected Ly$\alpha$ equivalent width and SFR/M* (97.5% confidence). These results imply a physical connection between the HI disk and the CGM, which is on scales an order-of-magnitude larger. This is consistent with the picture in which the HI disk is nourished by accretion of gas from the CGM.

==> figures.tex <==
\begin{figure}
\begin{center}
\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,scale=0.65,angle=-0]{f1.ps}  \\
\end{center}
\caption{Overview of the COS-GASS sample. The figure shows a representative galaxy from the COS-GASS sample at the center of the plot and QSO sightlines shown as filled circles. The sample consists of 45 QSO-galaxy pairs probing the CGM in galaxies from the GASS project. The stellar masses of the sample galaxies range between $\rm 10^{10.1-11.1}~M_{\odot}$. The median optical (R$\rm_{90}$) and \textsc{Hi} radii (R$\rm_{HI}$) of the galaxies in the sample are shown as blue and red ellipses respectively at the center of the plot. The physical size corresponding to the FWHM of the Arecibo beam at 21~cm at the average redshift for our sample ($\overline{z}=0.037$) is shown in yellow. The QSO sightlines cover a range of impact parameters from 63-231~kpc. The position of the QSO sightlines with respect to the foreground galaxy are shown as filled green circles. The orientations of sightlines with respect to the disks are estimated using position angle of the galaxy major axis from SDSS photometry. We consider galaxies with de Vaucouleurs a/b parameter greater than 0.7 as having a face-on orientation. These galaxies were assigned an orientation parameter of zero degrees and are identified in this figure with a lighter shade of green.}  
 \label{fig-sample} 
\end{figure}


\begin{figure}
\begin{center}
\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,scale=0.45,angle=-0]{f2a.ps}  \\
\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,scale=0.45,angle=-0]{f2b.ps} 
\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,scale=0.45,angle=-0]{f2c.ps}  \\
\end{center}
\caption{Top: Variation of \Lya equivalent widths as a function of impact parameter i.e. $\rm \rho$. The COS-GASS data are shown as circles and the COS-Halos data are shown as diamonds. The galaxies are divided into two bins based on their specific star-formation rates (see text for details). This is indicated by the color of the symbols. Blue and cyan indicate blue star-forming galaxies from the COS-GASS and COS-Halos samples respectively. Red and yellow indicate the red passive galaxies. As shown with the black line, the radial distribution of the \Lya equivalent width can be fit as exponential with an e-folding scale length of 136~kpc. The grey shaded region represents the uncertainty associated with the fit.
Bottom: Variation of \Lya equivalent widths with as a function of normalized impact parameter i.e. $\rm \rho/R_{vir}$. The panel on the left presents data using a logarithmic radial scale where as the one on the right is a linear radial scale. The best-fit exponential distribution is illustrated with the black solid line. The uncertainty associated with the fit is shown in grey. The best-fit parameters are  labeled at the  bottom of the right panel and imply an e-folding scale length of 0.85 $\rm R_{vir}$.}  
 \label{fig-rho_W} 
\end{figure}



\begin{figure}
\includegraphics[trim = 00mm 0mm 0mm 0mm, clip,scale=0.40, angle=-0]{f3a.ps}  
\includegraphics[trim = 00mm 0mm 25mm 0mm, clip,scale=0.65, angle=-0]{f3b.ps}   \\
\caption{ Left: 21~cm \textsc{Hi} spectra of one of our target galaxies from the GASS sample. This illustrates a typical \textsc{Hi} profile for our sample. The abscissa and ordinate show the velocity in the rest-frame of the galaxy and the flux in the 21~cm  \textsc{Hi} hyperfine transition. The part of the spectrum showing the emission is indicated with the grey shaded region.  The velocity centroid of the \Lya absorber detected in the CGM of this galaxy (at $\rho=$155~kpc) is marked in red. We term the offset between the centroid of the \Lya absorption feature and the systemic velocity of the galaxy (based on SDSS emission-line estimation) as $\delta\rm v_{Ly\alpha}$ (labeled as the red double headed arrow). Similarly the velocity extent of the \textsc{Hi} with respect to the systemic velocity of the galaxy is termed as $\delta\rm v_{HI}$ (marked as the blue double headed arrow). Since \textsc{Hi} profiles are not always symmetric with respect to the systemic velocity, we pick the velocity edge of the \textsc{Hi} profile that is closest to \Lya  centroid to estimate $\delta\rm v_{HI}$.  Right: Velocity centroid of \Lya absorbers as a function of the velocity width of the 21~cm \textsc{Hi} profile associated with the host galaxies. All the velocities are in the rest-frame of their host galaxies as measured by optical emission lines.  The full widths of the \Lya features are shown as the vertical bars passing the centroids marked by a filled circle. The color of each circle indicates the color of the galaxy as defined by their sSFR and presented in Table~1.}
 \label{fig-velocity}
\end{figure}


\begin{figure}[!h]
\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,scale=0.5,angle=-0]{f4a.ps}  
\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,scale=0.5,angle=-0]{f4b.ps}  \\
\caption{Left: \Lya equivalent width as a function of orientation of the QSO sightline with respect to the optical major axis of the galaxy. The open circles represents galaxies that are face-on and their orientation parameter set to zero. The color of the circles represents the color of the galaxy that was summarized in Table~1. Right: The excess in \Lya equivalent width ([Log W - $\rm \overline{Log~W}]_{Ly\alpha}$), which is independent of the impact parameter of the sightlines, as a function of orientation of the QSO sightlines with respect to the target galaxy. The dotted line corresponds to the expected equivalent width based on fit to Figure~2. We find no correlations between orientation and \Lya strengths. The face-on galaxies were excluded while measuring the strength of the correlation.}
\label{fig-Orientation} 
\end{figure}

\begin{figure}
\includegraphics[trim = 20mm 127mm 20mm 0mm, clip,scale=0.50,angle=-0]{f5a.ps} 
\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,scale=0.5,angle=-0]{f5b.ps} \\
\caption{Equivalent width of \Lya as a function of 21~cm \textsc{Hi} mass and the excess in \Lya equivalent width ([Log W - $\rm \overline{Log~W}]_{Ly\alpha}$), which is independent of impact parameter of the sightline, as a function of the \textsc{Hi} mass fraction $\rm M_{HI}/M_{\star}$ of the galaxies. The size of the \textsc{Hi} disk is indirectly estimated from the tight \textsc{Hi} size-mass relation \citep{swaters02}. We find statistically significant correlations with a statistical significance of 97.7\% in the left panel and 99.4\% in the right. The top x-axis of the left panel converts the \textsc{Hi} mass to a radius of the \textsc{Hi} disk (see text for details). The average equivalent widths derived from the stacked spectra (presented in the next figure) are plotted as green asterisk.} 
\label{fig-HI} 
\end{figure}



\begin{figure}
\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,scale=0.6,angle=-0]{f6a.ps} 
\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,scale=0.6,angle=-0]{f6b.ps} 
\caption{Composite \Lya absorption-lines stacked as a function of \textsc{Hi} mass and gas fraction ($\rm M(HI)/M_{\star}$). Individual \Lya absorbers were centered at their centroid of the feature i.e. $\rm v_{centroid}=0$~\kms,  and then added to produce the stacks. Each of the stacked spectra are composed of approximately 8-10 individual spectra in that labeled \textsc{Hi} mass range. The equivalent width and the peak depth (f$\rm_{peak}$) of the absorption features are labeled in the right corner of each plot in red.  These set of stacks are not corrected for impact parameter variations and consequently show a weaker trend just like the left panel of Figure~5. Similar plots with impact parameter bins are presented in the next figure. }
\label{fig-HIstacks} 
\end{figure}



\begin{figure}
\hspace{-0.75cm}
\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,scale=0.62,angle=-0]{f7a.ps} 
\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,scale=0.62,angle=-0]{f7b.ps} \\
\caption{Left: Stacks of \Lya absorption similar to those presented in Figure~\ref{fig-HIstacks} but with bins that divide the sample into subsets of impact parameter - one less than and the other greater than 170~kpc. The values for the bins were chosen such that the sample is divided more or less equally into 4 bins. Systematic variations the strength of the \Lya absorption as a function of \textsc{Hi} mass within each bin can be seen. The equivalent width of the features are labeled in the right corner of each plot in red.  Right: Stacks similar to those on the left, but binned by \textsc{Hi} mass fraction and  normalized impact parameter ($\rho/\rm R_{vir}$). The sample was divided along the median value of normalized impact parameter of 0.64.}
\label{fig-HIstacks_sub} 
\end{figure}


\begin{figure}
\includegraphics[trim = 0mm 130mm 0mm 20mm, clip,scale=0.5,angle=-0]{f8.ps}  \\
\caption{\Lya equivalent width as a function of the impact parameter  normalized by the radius of the \textsc{Hi} disk ($\rm \rho/R_{HI}$). The absorbers are shown as colored filled circles with their colors indicating the color of the galaxy as defined by their sSFR and presented in Table~1. Sightlines within about 6 $R_{HI}$ all produce strong saturated \Lya lines. In green we plot the covering fraction of strong \Lya absorbers with equivalent width larger than $\rm 0.32~\AA $~(-0.5~dex). This corresponds to a column density of  $\rm \approx 6 \times 10^{13}~cm^{-2}$ or larger. The right abscissa is labeled to indicate the scale.}  
 \label{fig-RHI} 
\end{figure}



 \begin{figure}[!h]
\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,scale=0.5,angle=-0]{f9a.ps}  
\includegraphics[trim = 0mm 0mm 0mm 0mm, clip,scale=0.5,angle=-0]{f9b.ps}    \\
\caption{Left:  Variation in the \Lya equivalent width as a function of SFR.  The absorbers are shown as colored filled circles with their colors indicating the color of the galaxy as defined by their sSFR and presented in Table~1. Right: The excess \Lya equivalent width as a function of specific SFR. The correlations have a statistical significance of only 91\% (left panel) and 97\% (right panel). These are weaker than the corresponding ones in Figure 5.}
 \label{fig-SFR} 
\end{figure}


 \clearpage
 
 
 
 
 
 
 
